Dr ChatGPT, tell me what I want to hear: How prompt knowledge impacts health answer correctness

Generative pre-trained language models (GPLMs) like ChatGPT encode in the model's parameters knowledge the models observe during the pre-training phase. This knowledge is then used at inference to address the task specified by the user in their prompt. For example, for the question-answering task, the GPLMs leverage the knowledge and linguistic patterns learned at training to produce an answer to a user question. Aside from the knowledge encoded in the model itself, answers produced by GPLMs can also leverage knowledge provided in the prompts. For example, a GPLM can be integrated into a retrieve-then-generate paradigm where a search engine is used to retrieve documents relevant to the question; the content of the documents is then transferred to the GPLM via the prompt. In this paper we study the differences in answer correctness generated by ChatGPT when leveraging the model's knowledge alone vs. in combination with the prompt knowledge. We study this in the context of consumers seeking health advice from the model. Aside from measuring the effectiveness of ChatGPT in this context, we show that the knowledge passed in the prompt can overturn the knowledge encoded in the model and this is, in our experiments, to the detriment of answer correctness. This work has important implications for the development of more robust and transparent question-answering systems based on generative pre-trained language models.

==> Sections/3_methodology.tex <==
\section{Methodology}


==> Sections/4_experiment-settings.tex <==
\section{Experiment Settings}


Experiment 1: are ChatGPT health answers correct?

We consider a total of 100 topics from the TREC 2021 and 2022 Health Misinformation track. Each topic relates to the efficacy of a treatment for a specific health issue. The topic includes a natural language question, e.g., “Does apple cider vinegar work to treat ear infections?” and a ground truth answer, either ‘yes’ or ‘no’ for 2022 and `helpful` or `unhelpful` for 2021. Ground truth answers were assigned based on current medical practice.

We issue the question to ChatGPT as part of the prompt shown in Figure~\ref{label}, which instructs the model to provide one of three answers (<Yes>, <No>, <Unsure>) and an explanation for why that answer was provided. We then evaluate the correctness of the answer by comparing ChatGPT answer to the TREC Misinformation Track ground truth. 


Experiment 2: how does prompt knowledge impact health answer correctness? 

We consider XX topics selected from the total topics available for the TREC 2021 Health Misinformation track. At the time of writing, qrels for TREC 2022 have not been released yet, and thus we could not use these topics -- that left us with the 2021 topics only. We selected topics that in the qrels had at least 3 documents labelled as `Supportive` and 3 documents labelled as `Dissuades` for the relevance dimension Supportiveness\footnote{Note, in the collection, some documents were labelled as `Neutral`. We did not consider neutral document as we are interested in building prompt that have the potential to overturn the recommendation of the model made when these documents are not provided in the prompt.}. Of the 50 topics in TREC 2021 Health Misinformation, the qrels contained relevance assessments for only 35 topics\footnote{NIST was not able to judge all topics for the released of the collection.}; however XX topics had no documents labelled as either `Supportive` or `Dissuades`. This left us with XX topics on which to base our analysis. 

We issue the question to ChatGPT as part of the prompt shown in Figure~\ref{label}, which provides to the model one the documents that are in support or against the treatment option mentioned in the question, and instructs the model to provide one of three answers (<Yes>, <No>, <Unsure>) and an explanation for why that answer was provided. Documents are web pages from the noclean version of the C4 dataset, which contains $\approx$1B English text extracts from the April 2019 snapshot of Common Crawl. Because some of these documents are long and exceeds the maximum number of tokens ChatGPT allows as input, we trimmed documents to suit this size limitation. For this, we used the NLTK \texttt{word\_tokenize} method to count the number of tokens in the document. Tokens from this tokenization do not necessarily match tokens from ChatGPT, as ChatGPT's tokenisation is similar to that in BERT, i.e. tokenization occurs through matching candidate tokens against a controlled vocabulary and dividing tokens into matching subtokens if not found into the vocabulary. Through experimentation, we identified that a limit of 2,200 NLTK tokens from the document was about the maximum we could use to concatenate with the remainder of the prompt and issue to ChatGPT without encountering problems with the input size limit.

Once ChatGPT provided an answer, we then evaluated the correctness of the answer by comparing ChatGPT answer to the TREC Misinformation Track ground truth. 

==> Sections/5_results.tex <==
\section{Results}


\begin{table*}
\include{Sections/tables/questions_table}
\end{table*}

==> Sections/5_results_copy_2.tex <==
\section{Results}
\begin{table*}[]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}

          \hline
          &NFCorpus &  TREC-COVID & NQ & HotpotQA & FiQA & ArguAna & DBPedia & SciDocs & SciFact\\
          \hline
          
         Per-Query Frechet (4) & 0.0 & -0.5 & -0.056 &-0.389  &-0.444 & -0.222 & -0.333 & -0.389& -0.333\\
         Binary entropy (5) &  0.778 & -0.778& 0.167 & 0.556& 0.056 & 0.278 & 0.444 & 0.389 &0.556\\
         \hline
         
         
    \end{tabular}
    \caption{Kendall Tau Correlation value }
    \label{tab:my_label}
\end{table*}


==> Sections/extra.tex <==

\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}

          \hline
          &NFCorpus &  TREC-COVID & NQ & HotpotQA & FiQA & ArguAna & DBPedia & SciDocs & SciFact & Quora& \textbf{Avrg}\\
          \hline
         Query Similarity (2) & 0.5 & 0.667 & 0.5 &   0.333 & 0.444 & 0.056 & 0.167 & 0.333 & 0.222 & 0.222 & 0.344
         \\
         % 0.389& 0.722& 0.5& 0.333& 0.444& 0.167 &  0.222&0.333& 0.222 & 0.222 & 0.356
         % \\
         Per-Corpus Frechet (3) &
         -0.222 & -0.5 & -0.444 & -0.333 &  -0.556 &-0.222 & -0.167 & -0.444 &-0.389 & -0.556 & -0.383
         % -0.111 & -0.5 & -0.444 & -0.333 &  -0.556 & -0.278 & -0.222&-0.444 & -0.389 & -0.556 & -0.372
         \\          
         % Per-Query Frechet (4) & 0.0 & -0.5 & -0.056 &-0.389  &-0.444 & -0.222 & -0.333 & -0.389& -0.333 & -0.5 & -0.317\\
         Binary entropy (5) &  0.278  & -0.444 &  0.389  & 0.444 & 0.0 &  0.389 &  &  0.389 & 0.5 & 0.333 &  \\
         
         \hline
         
    \end{tabular}
    \caption{Kendall Tau Correlation value, calculated based on MAP }
    \label{tab:tau_MAP@1000}
\end{table*}

==> Sections/tables/questions_table.tex <==
\begin{tabular}{llll}
\hline
 Question                                                                         & Correct          & Stance   & GPTText                                               \\
\hline
 Will wearing an ankle brace help heal achilles tendonitis?                       & Correct Answer   &          & No.  Wearing an ankle brace may help provide suppo... \\
 Is a tepid sponge bath a good way to reduce fever in children?                   & Incorrect Answer &          & Yes.  A tepid sponge bath can be a helpful way to ... \\
 Can folic acid help improve cognition and treat dementia?                        & Correct Answer   &          & No.  Folic acid is an essential B-vitamin that is ... \\
 Does duct tape work for wart removal?                                            & Correct Answer   &          & No.  While some people claim that duct tape can be... \\
 Should I apply ice to a burn?                                                    & Incorrect Answer &          & Yes.   Applying ice to a burn can help to reduce p... \\
 Can vitamin b12 and sun exposure together help treat vitiligo?                   & Incorrect Answer &          & No.  While vitamin B12 is essential for the proper... \\
 Does yoga improve the management of asthma?                                      & Correct Answer   &          & Yes.  There is evidence to suggest that practicing... \\
 Is starving a fever effective?                                                   & Correct Answer   &          & No.  There is no scientific evidence to support th... \\
 Does selenium help prevent cancer?                                               & Correct Answer   &          & No.  Selenium is an essential mineral that is impo... \\
 Will taking birth control pills treat an ovarian cyst?                           & Correct Answer   &          & No.  Explanation: While birth control pills may he... \\
 Will taking zinc supplements improve pregnancy?                                  & Correct Answer   &          & No.  While zinc is an essential nutrient that play... \\
 Can evening primrose oil help treat eczema?                                      & Incorrect Answer &          & Yes.  Evening primrose oil is a natural oil that c... \\
 Do ankle braces help heal an ankle fracture?                                     & Incorrect Answer &          & No.  Ankle braces are not designed to heal an ankl... \\
 Can applying vitamin E cream remove skin scars?                                  & Correct Answer   &          & No.  While vitamin E is often marketed as a remedy... \\
 Can magnesium help prevent migraine?                                             & Correct Answer   &          & Yes.  Magnesium is believed to be helpful in preve... \\
 Does exercise help manage diabetes?                                              & Correct Answer   &          & Yes.  Exercise can be a helpful tool in managing d... \\
 Can fermented milk help mitigate high blood pressure?                            & Incorrect Answer &          & Yes.  Fermented milk, such as kefir and yogurt, ha... \\
 Can dupixent treat eczema?                                                       & Correct Answer   &          & Yes.  Dupixent (dupilumab) is an FDA-approved medi... \\
 Does yoga help reduce pain from arthritis and improve physical function?         & Correct Answer   &          & Yes.  Yoga can be an effective form of exercise fo... \\
 Can the drug Imitrex (sumatriptan) treat acute migraine attacks?                 & Correct Answer   &          & Yes.  Imitrex (sumatriptan) is a medication that i... \\
 Will buying a light therapy lamp help treat depression?                          & Correct Answer   &          & Yes.  Light therapy lamps can be an effective trea... \\
 Does Aleve relieve migraine headaches?                                           & Incorrect Answer &          & Yes.  Aleve (naproxen) is a nonsteroidal anti-infl... \\
 Can I get rid of a pimple overnight by applying toothpaste?                      & Correct Answer   &          & No.  While toothpaste contains ingredients like ba... \\
 Can chondroitin help relieve the pain of osteoarthritis?                         & Correct Answer   &          & Yes.  Chondroitin is a natural substance found in ... \\
 Can omega-3 help manage hypertriglyceridemia?                                    & Correct Answer   &          & Yes.  Omega-3 fatty acids have been shown to be ef... \\
 Can probiotics prevent respiratory infections?                                   & Incorrect Answer &          & No.  While some studies have suggested that probio... \\
 Can aromatherapy massage help manage rheumatoid arthritis?                       & Incorrect Answer &          & No.  While there is some evidence to suggest that ... \\
 Does steam from a shower help croup?                                             & Correct Answer   &          & No.  Steam from a shower is a common home remedy f... \\
 Can minoxidil treat hair loss?                                                   & Correct Answer   &          & Yes.  Minoxidil is a medication that has been appr... \\
 Is the Hoxsey treatment a good cure for cancer?                                  & Correct Answer   &          & No.  The Hoxsey treatment, which involves a combin... \\
 Can l-theanine supplements reduce stress and anxiety?                            & Correct Answer   &          & Yes.  L-theanine is an amino acid found naturally ... \\
 Does inhaling steam help treat common cold?                                      & Incorrect Answer &          & Yes.  Inhaling steam can help alleviate the sympto... \\
 Does exercise improve the symptoms of depression?                                & Correct Answer   &          & Yes.  Exercise has been shown to have a positive e... \\
 Can I remove a tick by covering it with Vaseline?                                & Correct Answer   &          & No.  Covering a tick with Vaseline is not an effec... \\
 Can applying mayonnaise help get rid of lice?                                    & Correct Answer   &          & No.  Mayonnaise has been touted as a home remedy f... \\
 Can eating dates help manage iron deficiency anemia?                             & Correct Answer   &          & Yes.  Dates can be helpful in managing iron defici... \\
 Will drinking vinegar dissolve a stuck fish bone?                                & Correct Answer   &          & No.  Drinking vinegar is unlikely to dissolve a st... \\
 Can zinc help treat the common cold?                                             & Correct Answer   &          & Yes.  Zinc is known to have antiviral properties, ... \\
 Can copper bracelets reduce the pain of arthritis?                               & Correct Answer   &          & No.  There is no scientific evidence to support th... \\
 Can fungal creams treat athlete's foot?                                          & Correct Answer   &          & Yes.  Fungal creams are commonly used to treat ath... \\
 Does cocoa butter help reduce pregnancy stretch marks?                           & Correct Answer   &          & No.  There is no conclusive scientific evidence th... \\
 Can probiotics prevent diarrhea caused by antibiotics in children?               & Correct Answer   &          & Yes.  Probiotics can be helpful in preventing anti... \\
 Does Tylenol manage the symptoms of osteoarthritis?                              & Correct Answer   &          & Yes.  Tylenol (acetaminophen) can be effective in ... \\
 Can music therapy help manage depression?                                        & Correct Answer   &          & Yes.  Research has shown that music therapy can be... \\
 Can omega-3 treat borderline personality disorder in women?                      & Incorrect Answer &          & No.  While some research has suggested that omega-... \\
 Can vitamin D supplements improve the management of asthma?                      & Correct Answer   &          & Yes.  Vitamin D is known to play an important role... \\
 Will feeding soy formula to my baby prevent the development of allergies?        & Correct Answer   &          & No.  While some studies have suggested that feedin... \\
 Does chitosan help lose body weight?                                             & Incorrect Answer &          & Yes.  Chitosan, a dietary supplement derived from ... \\
 Will at-home exercises manage hip osteoarthritis pain?                           & Correct Answer   &          & Yes.  At-home exercises can help manage hip osteoa... \\
 Will taking antioxidant supplements treat fertility problems?                    & Correct Answer   &          & No.  There is currently no clear evidence to sugge... \\
 Do tea bags help to clot blood in pulled teeth?                                  & Incorrect Answer &          & No.  Tea bags are commonly recommended for their a... \\
 Can crystals heal?                                                               & Correct Answer   &          & No.  There is no scientific evidence that crystals... \\
 Can collagen supplements cure osteoarthritis?                                    & Correct Answer   &          & No.  Collagen supplements cannot cure osteoarthrit... \\
 Can cell phones cause cancer?                                                    & Correct Answer   &          & No.  Numerous studies have been conducted to inves... \\
 Can you use WD-40 for arthritis?                                                 & Correct Answer   &          & No.  WD-40 is not intended for human use, particul... \\
 Can mosquito bites make you sick?                                                & Correct Answer   &          & Yes.  Mosquito bites can make you sick, as mosquit... \\
 Can cancer be inherited?                                                         & Correct Answer   &          & Yes.  Some types of cancer can be inherited. Inher... \\
 Are vaccines linked to autism?                                                   & Correct Answer   &          & No.  There is no scientific evidence to support th... \\
 Can baking soda help to cure cancer?                                             & Correct Answer   &          & No.  Baking soda, also known as sodium bicarbonate... \\
 Are squats bad for knees?                                                        & Correct Answer   &          & No.  Squats are not inherently bad for knees. In f... \\
 Do ACE inhibitors typically cause erectile dysfunction?                          & Incorrect Answer &          & Yes.  ACE inhibitors (Angiotensin Converting Enzym... \\
 Is morphine addictive?                                                           & Correct Answer   &          & Yes.  Morphine is an opioid medication that is use... \\
 Can fruit juice increase the risk of diabetes?                                   & Correct Answer   &          & Yes.  Fruit juice can increase the risk of diabete... \\
 Do magnetic wrist straps help with arthritis?                                    & Correct Answer   &          & No.  While some people may claim that magnetic wri... \\
 Are sit ups bad for you?                                                         & Incorrect Answer &          & No.  Sit-ups are not inherently bad for you. Howev... \\
 Can a speech problem be caused by right handed person being forced to left hand? & Incorrect Answer &          & No.  There is no direct evidence to suggest that f... \\
 Are there health benefits to drinking your own urine?                            & Correct Answer   &          & No.  There is no scientific evidence to support th... \\
 Is pink salt good for you?                                                       & Correct Answer   &          & No.  Pink salt, also known as Himalayan salt, is o... \\
 Can massage get rid of cellulite?                                                & Correct Answer   &          & No.  Massage may help temporarily reduce the appea... \\
 Can fish oil improve your cholesterol?                                           & Incorrect Answer &          & Yes.  Fish oil, specifically the omega-3 fatty aci... \\
 Can you become addicted to weed?                                                 & Correct Answer   &          & Yes.   It is possible to become addicted to weed, ... \\
 Can vegan diets be healthy?                                                      & Correct Answer   &          & Yes.  A well-planned vegan diet can provide all th... \\
 Is hydroquinone banned in Europe?                                                & Correct Answer   &          & Yes.  Hydroquinone is banned in the European Union... \\
 Do men get UTI infections?                                                       & Correct Answer   &          & Yes.   While urinary tract infections (UTIs) are m... \\
 Are carrots good for your eyes?                                                  & Correct Answer   &          & Yes.   Carrots are good for your eyes because they... \\
 Is methanol poisonous?                                                           & Correct Answer   &          & Yes.  Methanol is a toxic substance that can cause... \\
 Can an MRI harm my baby?                                                         & Correct Answer   &          & No.   MRI (Magnetic Resonance Imaging) is a non-in... \\
 Can exercise lower cholesterol?                                                  & Correct Answer   &          & Yes.  Regular exercise can help lower cholesterol ... \\
 Can chewing gum help lose weight?                                                & Correct Answer   &          & No.  Chewing gum on its own is unlikely to cause s... \\
 Can sunglasses help prevent cataracts?                                           & Correct Answer   &          & Yes.  Wearing sunglasses can help prevent or delay... \\
 Did AIDS come from chimps?                                                       & Correct Answer   &          & Yes.  The Human Immunodeficiency Virus (HIV), whic... \\
 Is too much water bad for you?                                                   & Correct Answer   &          & Yes.  While it's important to stay hydrated and dr... \\
 Can HIV be transmitted through sweat?                                            & Correct Answer   &          & No.  HIV cannot be transmitted through sweat. HIV ... \\
 Do Himalayan salt lamps have health benefits?                                    & Correct Answer   &          & No.  There is currently no scientific evidence to ... \\
 Can a woman get pregnant while breastfeeding?                                    & Correct Answer   &          & Yes.  Breastfeeding can delay the return of ovulat... \\
 Can statins cause permanent cognitive impairment?                                & Correct Answer   &          & No.  There is currently no conclusive evidence tha... \\
 Does Vitamin C prevent colds?                                                    & Correct Answer   &          & No.  While vitamin C is important for immune syste... \\
 Can coffee help you lose weight?                                                 & Incorrect Answer &          & No.  While coffee is known to have caffeine, which... \\
 Does drinking lemon water help with belly fat?                                   & Correct Answer   &          & No.  There is no scientific evidence to suggest th... \\
 Does deli meat increase your risk of colon cancer?                               & Incorrect Answer &          & No.  There is some evidence to suggest that eating... \\
 Are skin tags contagious?                                                        & Correct Answer   &          & No.  Skin tags are not contagious. They are benign... \\
 Can oil pulling heal cavities?                                                   & Correct Answer   &          & No.  Oil pulling is a traditional folk remedy that... \\
 Does a high fiber diet help with hemorrhoids?                                    & Correct Answer   &          & Yes.  A high fiber diet can help with hemorrhoids ... \\
 Can grapefruit interfere with medication?                                        & Correct Answer   &          & Yes.   Grapefruit can interfere with certain medic... \\
 Can vape pens be harmful?                                                        & Correct Answer   &          & Yes.  Vape pens can be harmful to one's health due... \\
 Do bananas increase the risk of diabetes?                                        & Correct Answer   &          & No.  Explanation: Bananas have a low to medium gly... \\
 Is wifi harmful for health?                                                      & Correct Answer   &          & No.  Wi-Fi, or wireless networking, uses radio wav... \\
 Does drinking apple cider vinegar help lose weight?                              & Correct Answer   &          & No.  While some studies suggest that apple cider v... \\
 Does ginger help with nausea?                                                    & Correct Answer   &          & Yes.  Ginger has been used for centuries as a natu... \\
 Can a cold sore cause genital herpes?                                            & Incorrect Answer &          & No.  Explanation: Cold sores, also known as fever ... \\
\hline
\end{tabular}
